An Energy Conserving Vlasov Solver That Tolerates Coarse Velocity Space Resolutions: Simulation of MMS Reconnection Events

Vlasov solvers that operate on a phase-space grid are highly accurate but also numerically demanding. Coarse velocity space resolutions, which are unproblematic in particle-in-cell (PIC) simulations, can lead to numerical heating or oscillations in standard continuum Vlasov methods. We present a new dual Vlasov solver which is based on an established positivity preserving advection scheme for the update of the distribution function and an energy conserving partial differential equation solver for the kinetic update of mean velocity and temperature. The solvers work together via moment fitting during which the maximum entropy part of the distribution function is replaced by the solution from the partial differential equation solver. This numerical scheme makes continuum Vlasov methods competitive with PIC methods concerning computational cost and enables us to model large scale reconnection in Earth's magnetosphere with a fully kinetic continuum method. The simulation results agree well with measurements by the MMS spacecraft.

==> spatial_coupling.tex <==

In large-scale simulations, for example of magnetospheres, it is common
that some areas need kinetic treatment while others are represented
well by a much cheaper fluid model. Since it is not possible to
do fully kinetic simulations of such systems, a good approach is
to use kinetic models only where necessary and use fluid models
elsewhere. At the interfaces between the two models, they
must then provide appropriate boundary information for each other.
In this section we describe a method how to smoothly couple
the Vlasov solver to the ten-moment fluid solver (the
translation to coupling of Vlasov and five-moment solvers
is straightforward).

\begin{algorithm}[H]\label{alg:boundary_moment_fitting}
\SetAlgoLined
  \KwIn{Ten-moment boundary data $n_{\text{bd}}^i$, $\mathbf{u}_{\text{bd}}^i$, $\mathcal{P}_{\text{bd}}^i$ in each boundary cell $i$}
  \KwOut{Distribution function $f_{\text{bd}}^i$ in each boundary cell $i$}
  \Boundarymomentfitting{}{
  \For{$i\ \mathrm{in\ boundary\ cells}$}{
    Constant extrapolation of the distribution function at the border into the boundary cells: $f_{\text{bd}}^i = f_{\text{border}}$\\
    Calculate moments $n_{\text{V}}^i$, $\mathbf{u}_{\text{V}}^i$, $\mathcal{P}_{\text{V}}^i$ from $f_{\text{bd}}^i$\\
    Rescale the distribution function $f_{\text{bd}}^i$ and its moments $n_{\text{V}}^i$, $\mathbf{u}_{\text{V}}^i$, $\mathcal{P}_{\text{V}}^i$ by
    $n_{\text{F}}^i/n_{\text{V}}^i$ to match the fluid density\\
    Calculate ten-moment Maxwellian $f_{\text{M,V}}^i$ from $n_{\text{V}}^i$, $\mathbf{u}_{\text{V}}^i$, $\mathcal{P}_{\text{V}}^i$\\
    Calculate ten-moment Maxwellian $f_{\text{M,F}}^i$ from the fluid solver's moments\\
    Exchange ten-moment Maxwellians: $f_{\text{bd}}^i = f_{\text{bd}}^i - f_{\text{M,V}}^i + f_{\text{M,F}}^i$\\
    Limit $f_{\text{bd}}^i$
  }
  }
 \caption{Distribution function from ten-moment boundary data}
\end{algorithm}


The fluid model needs information on the distribution function's
moments. Those can be easily provided by the Vlasov model that
has the full distribution function available. The route from
fluid to Vlasov is more challenging because there is not one
unique distribution function that fits a set of given
moments. We can, however, assume that the
shape of the distribution function does not significantly
change within a few cells and start with an extrapolation
of the distribution function into the boundary cells.
Then it is adapted to fit the moments
given by the fluid solver boundary data. This has
been first done by \cite{rieke-trost-grauer:2015} with
a different moment fitting method.

Algorithm~\ref{alg:boundary_moment_fitting} shows the necessary steps
for calculating the distribution function in the boundary cells with
moment fitting. The primary difference compared to the procedure
in Algorithm~\ref{alg:timestep} is that now the distribution function
is rescaled to match the density provided by the boundary data.


